Beyond Sharing: Conflict-Aware Multivariate Time Series Anomaly Detection

Massive key performance indicators (KPIs) are monitored as multivariate time series data (MTS) to ensure the reliability of the software applications and service system. Accurately detecting the abnormality of MTS is very critical for subsequent fault elimination. The scarcity of anomalies and manual labeling has led to the development of various self-supervised MTS anomaly detection (AD) methods, which optimize an overall objective/loss encompassing all metrics' regression objectives/losses. However, our empirical study uncovers the prevalence of conflicts among metrics' regression objectives, causing MTS models to grapple with different losses. This critical aspect significantly impacts detection performance but has been overlooked in existing approaches. To address this problem, by mimicking the design of multi-gate mixture-of-experts (MMoE), we introduce CAD, a Conflict-aware multivariate KPI Anomaly Detection algorithm. CAD offers an exclusive structure for each metric to mitigate potential conflicts while fostering inter-metric promotions. Upon thorough investigation, we find that the poor performance of vanilla MMoE mainly comes from the input-output misalignment settings of MTS formulation and convergence issues arising from expansive tasks. To address these challenges, we propose a straightforward yet effective task-oriented metric selection and p&s (personalized and shared) gating mechanism, which establishes CAD as the first practicable multi-task learning (MTL) based MTS AD model. Evaluations on multiple public datasets reveal that CAD obtains an average F1-score of 0.943 across three public datasets, notably outperforming state-of-the-art methods. Our code is accessible at https://github.com/dawnvince/MTS_CAD.

==> NewMethod.tex <==
\section{Methodology}
\label{sec:model}
In this section, we first give an overview of the system. Then we introduce the sub-components of the model individually, including task-oriented feature selection, expert network, personalized \& shared gate and tower network. At last, we introduce the loss balance module.
\subsection{Overall Structure}
As illustrated in Fig. \ref{Fig.model}, we leverage a group of task-oriented isolated structures to tackle the conflict problems discussed in Section~\ref{sec: introd}. Since previous works have no independent structures to determine whether inter-metric dependencies are helpful or harmful to a specific metric, the correlation may have a negative impact on describing reasonable patterns of the current metric. Our approach, as each task has its own structure to autonomously select various expert-derived features that are highly correlated with it, solves the conflicts in an elegant manner. Moreover, the isolated tower becomes even more focused on its own metric since irrelevant information is separated out.
% Since the unified model has no explicit structure for isolation, the correlation may have a negative impact on describing reasonable patterns. Metric-level multi-task oriented framework, as each task has its own structure in the vicinity of the output layer, solves the conflict in an elegant manner while maintaining the ability to capture inter-metric dependency by the former shared structure.

However, original frameworks like MMoE are unacclimatized when facing MTS issues. Firstly, \textbf{misalignment of input and output spaces} distract the gates from focusing on more relevant patterns. Secondly, well-designed structures are required to capture the complicated temporal-spatial dependency. Thirdly, massive metrics bring more interference to feature extraction, which needs a way for experts to \textbf{converge on specific traits}.

To address the problems mentioned above, we design CAD, a hierarchical unsupervised and forecasting-based model.
% Fig. \ref{Fig.model} illustrates the overall architecture of CAD. 
Then a two-dimensional input window is fed into multiple expert networks including a convolution layer to enrich the representation of temporal and inter-metric dependency (Section~\ref{subsec: expert}). The hybrid gating mechanism (Section~\ref{subsec: psgate}), which is designed for massive metrics, transforms the feature space selected for each metric (Section~\ref{subsec: feature select}) into a set of weights to fuse embeddings extracted by different experts. The embedding is then sent to its corresponding tower network (Section~\ref{subsec: tower}). All towers jointly finalize anomaly scores based on the gap between predictions and ground-truth values. For the multiple losses balance problem, we preprocess the data to balance all metrics' losses (Section~\ref{subsec: balance}). These components are then described in detail.


\subsection{Task-oriented Feature Selection}
\label{subsec: feature select}
In a typical scenario where MMoE works, there is no obvious correlation between the downstream task and the input data. In other words, each dimension of the input data is equally significant for the current task, thus each gate calculates the weight combination of experts based on all input data. This assumption, however, does not hold true in MTS anomaly detection. In this case, for a subtask determining if the particular metric is abnormal, it is counterintuitive that historical information in \textbf{its own feature space} is as important as the one in \textbf{overall input feature spaces} composed of other metrics. More metrics mean more possibility to distract the limited volume structure, especially when conflicts and reasonable drifts exist among metrics (discussed in Section~\ref{sec: drift}). We split the input at metric level, using its own \textbf{local} time window instead of \textbf{all} metrics' windows to prompt gate structure for learning personalized mappings from time series to distribution over experts. Hence the prediction of metric $k$ at time $t$ is:
$$
y_t^k = h_k(G_k(\mathbf{w_t^k}) \odot F(\mathbf{w_t}))
$$
where $\mathbf{w_t^k}$ denotes time window of the k-th metric in $\mathbf{w_t}$ defined in Section 3.1 and $F(\mathbf{w_t})$ denotes the output of expert networks.

\subsection{Expert Network}
\label{subsec: expert}
Expert networks are the main structure for extracting ample traits in time series. Each expert consists of one convolution layer and two feed-forward layers. Previous works primarily use RNN-based units, e.g. LSTM or GRU, to capture temporal patterns~\cite{omni, madgan, dvgcrn}. Whereas, its inherently sequential nature makes it impossible for parallel computation, dramatically increasing training time. By contrast, convolution network, known as a structure with superior computational parallelism, shows its powerful capability of extracting features in time series tasks~\cite{tcn, lstnet, dsanet}. Especially, kernels can sharpen the change within a successive region, which suits MTS anomaly detection tasks even better. 

In our implementation shown in Fig. \ref{Fig.expert}, the convolution layer contains $N$ kernels of width $l$ (equals to window size) and height 1. As a kernel sweeps through the input $\mathbf{w_t}$ including $K$ metrics, each metric's window is convolved into a single value, so the layer produces a vector whose size is $N\times1\times K$. In this way, we obtain temporal dependency by the metric-level convolution operation, meanwhile obtaining inter-metric dependency by the shared filters. Then the vector is flattened and further fed into a two-layer fully-connected network, forming an embedding of the original input. All embeddings constitute a candidate set.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/expert.png}
    \caption{Expert Network.}
    \label{Fig.expert}
\end{figure}

\subsection{Personalized \& Shared Gate}
\label{subsec: psgate}
A hybrid gate structure is employed to map the selected input to the weights of embeddings in the candidate set. If patterns of metrics differ greatly from each other, instead of sharing the same expert, the loss of backpropagation will induce them to take advantage of different experts, which is reflected by diverse weight combinations given by gates. This empowers the model to resolve conflicts and irrelevant drifts among metrics. Furthermore, we design a dual-gate mechanism. A shared gate $G_s$ receives all selected windows from input, yet a personalized gate $G_p^k$ belonging to the k-th metric only receives its own window. Since there are massive metrics, too many gates with the same weight make the backpropagation gradient more chaotic for experts. A shared gate with a greater weight can learn the robust mapping relationships between expert fusion and input from more data and is more likely to induce experts to converge on dominant characteristics. We combine shared gate and personalized gate to leverage the advantages of both, making personalized gate act as an auxiliary role to tune the subtle differences between metrics. The hybrid gate is formulated as follows:
$$
G_s(\mathbf{w_t^k}) = W_s\mathbf{w_t^k},\quad\, G_p^k(\mathbf{w_t^k}) = W_{pk}\mathbf{w_t^k},
$$
$$
G_k(\mathbf{w_t^k}) = softmax(\varepsilon \cdot G_s + (1-\varepsilon)\cdot G_p^k).
$$
where $W_s$ and $W_{pk}$ ($k=1,2,\cdots,M$) are trainable matrixs, and $\varepsilon > 0.5$ is a weight coefficient of the shared gate.
\subsection{Tower Network}
\label{subsec: tower}
In our framework, the purpose of the tower network is to condense the embeddings into one final predicted value. We utilize two dense layers along with activation function $ReLU$ and a dropout layer to reduce the dimensions. All towers' predictions are appended to set $\mathbf{\hat{y_t}}$. As the ground truth observation at time $t$ is $\mathbf{y_t}$, the final training objective aims to minimize $||\mathbf{y_t} - \mathbf{\hat{y_t}}||_2$ ($||\cdot||_2$ denotes L2-norm), which is also used in inference phase as anomaly score.

\subsection{Loss Balancing}
\label{subsec: balance}
Balancing the weight of loss for each metric is a crucial topic as improper weights could narrow the perspective of detection and neglect some important metrics. Thanks to the homogeneity among metrics and even between inputs and outputs in MTS anomaly detection, we are able to alleviate the problem of imbalance simply by proper data preprocessing. For datasets whose metrics are not on the same order of magnitude, we normalize the original training data via a MinMax Scaler. Hence the loss of metric won't be too far from each other. More details about data preprocessing can be found in Section \ref{sec: data}.
